Learning Representations and Generative Models for 3D Point Clouds

Three-dimensional geometric data offer an excellent domain for studying representation learning and generative modeling. In this paper, we look at geometric data represented as point clouds. We introduce a deep AutoEncoder (AE) network with state-of-the-art reconstruction quality and generalization ability. The learned representations outperform existing methods on 3D recognition tasks and enable shape editing via simple algebraic manipulations, such as semantic part editing, shape analogies and shape interpolation, as well as shape completion. We perform a thorough study of different generative models including GANs operating on the raw point clouds, significantly improved GANs trained in the fixed latent space of our AEs, and Gaussian Mixture Models (GMMs). To quantitatively evaluate generative models we introduce measures of sample fidelity and diversity based on matchings between sets of point clouds. Interestingly, our evaluation of generalization, fidelity and diversity reveals that GMMs trained in the latent space of our AEs yield the best results overall.

==> tables/post_rebuttal/generator_in_voxels_ae_2.tex <==
%!TEX root = ../../00-supplementary.tex
% \begin{table}[htb]
%     \small
%     \centering
%     \begin{tabularx}{\columnwidth}{C{1.7} C{.8} C{.9} C{.9} C{.9} C{.8}}
%         \hline
%         Metric  & [1] & [2] & [3] & [4] & [5]
%         \\
%         \hline
%         \hline
%         MMD-CD  & 0.0046 & 0.0025  & 0.0025  &0.0024 & \bf{0.0018}\\
%         MMD-EMD & 0.0915 & 0.0742  & 0.0729  &0.0750  & \bf{0.0651}\\
%         COV-CD  & 19.6   & 63.5    & 60.3    &60.9   & 68.9\\
%         COV-EMD & 22.4   & 66.6    & 64.8    &64.7   & 67.4\\
%         \hline
%     \end{tabularx}
%     \caption{MMD and Coverage metrics evaluated on the output of voxel-based methods at resolutions $32^3$ and $64^3$ and (oct-tree based) $128^3$, matched against the chair \emph{test set}, using the same protocol as in Table~3 of the main paper. Comparing: [1]~``raw'' $64^3$-voxel GAN \cite{wu2016_learning-a-probabilistic-latent-space}, [2]~latent $32^3$-voxel GMM-32, [3]~latent $64^3$-voxel GMM-32, [4]~latent $128^3$-octtree GMM-32, [5]~latent point-cloud GMM-32. Our volumetric models use 64-dimensional latent codes, and GMM-32 stands for a GMM with 32 full-covariance Gaussian components. For the mesh conversion we used the marching cubes algorithm (\citep{Lewiner03efficientimplementation}) with an iso-surface value of $0.5$. The rightmost column shows the results with our point-cloud based GMM.}
%     \label{table:latent_voxel_generators}
% \end{table}


\begin{table}[htb]
    \small
    \centering
    \begin{tabularx}{\columnwidth}{C{.2} C{1.2} C{1.4} C{1.} C{1.2}}
        \hline
        {}    & MMD-CD     & MMD-EMD   & COV-CD & COV-EMD \\
        \hline
        \hline
        A & 0.0025     & 0.0742      & 63.5   & 66.6\\
        B & 0.0024     & 0.0750      & 60.9   & 64.7     \\
        C & \bf{0.0018}& \bf{0.0651} & \bf{68.9}   & \bf{67.4}     \\
        \hline
    \end{tabularx}
    \caption{MMD and Coverage metrics evaluated on the output of voxel-based methods at resolutions $32^3$ and {\bf oct-tree based} $128^3$, matched against the chair \emph{test set}, using the same protocol as in Table~5 of the main paper. Comparing: A:~latent $32^3$-voxel GMM-32, B:~latent $128^3$-octtree GMM-32, C:~latent point-cloud GMM-32. Our volumetric models use 64-dimensional latent codes. GMM-32 stands for a GMM with 32 full-covariance Gaussian components. For the mesh conversion we used the marching cubes algorithm (\citep{Lewiner03efficientimplementation}) with an isovalue of $0.5$.}
    \label{table:latent_voxel_generators_2}
\end{table}

